The Effect of Noise Level on Causal Identification with Additive Noise Models

In recent years a lot of research has been conducted within the area of causal inference and causal learning. Many methods have been developed to identify the cause-effect pairs in models and have been successfully applied to observational real-world data in order to determine the direction of causal relationships. Many of these methods require simplifying assumptions, such as absence of confounding, cycles, and selection bias. Yet in bivariate situations causal discovery problems remain challenging. One class of such methods, that also allows tackling the bivariate case, is based on Additive Noise Models (ANMs). Unfortunately, one aspect of these methods has not received much attention until now: what is the impact of different noise levels on the ability of these methods to identify the direction of the causal relationship. This work aims to bridge this gap with the help of an empirical study. For this work, we considered bivariate cases, which is the most elementary form of a causal discovery problem where one needs to decide whether X causes Y or Y causes X, given joint distributions of two variables X, Y. Furthermore, two specific methods have been selected, \textit{Regression with Subsequent Independence Test} and \textit{Identification using Conditional Variances}, which have been tested with an exhaustive range of ANMs where the additive noises' levels gradually change from 1% to 10000% of the causes' noise level (the latter remains fixed). Additionally, the experiments in this work consider several different types of distributions as well as linear and non-linear ANMs. The results of the experiments show that these methods can fail to capture the true causal direction for some levels of noise.

==> chapters/overview.tex <==
\parencite[][]{janzing2012identifying}
\begin{enumerate}
	\item Method for inferring the existence of a latent common cause
	\item In practical applications they propose to prefer the causal hypothesis $X \to Y$
	      already iif the variance of $N_x$ is small compared to the variance of $N_y$ after
	      normalizing both $X$ and $Y$ to variance 1.
	\item they work with an assumption: let the variances of the noise terms $N_x$ and $N_y$ be
	      small compared to the curvature of the graph $(u(t),v(t))$, where
		$$X = u(t) + N_x$$ and $$Y = v(t) + N_y$$ and $$t\:confounder$$
	\item With this assumption and two other assumptions they define a limit and then provide
	      a proof that a CAN model becomes identifiable in this particular limit. They also expect
	      a stronger statement to hold but left this as future work (Need to further check other
	      papers which cite this one)
	\item They only addressed the low noise regime but expect the proposed model to work even
	      for strong noise, although in that case more data points are needed.
\end{enumerate}

\parencite[][]{hoyer2008nonlinear}
\begin{enumerate}
        \item Extends identifiability from linear non-gaussian to non-linear non-gaussian
	\item Furthermore, non-linear gaussian is also identifiable
	\item in their experiments they used different types of distributions, i.e., sub-gaussian
	      and super-gaussian but no experiments are done on the level of noise 
	      (variance / standard deviation)
	\item Their simple nonlinear model with independent additive noise is not consistent with the
	      data in either (e.g. using time shift on data by one time step)
	\item (need to find code)
\end{enumerate}

\parencite[][]{hu2018causal}
\begin{enumerate}
        \item generalizes ANM to a mixture model, which consists of a finite number of ANMs
  and provides the condition of its causal identifiability
	\item Clustering underlying generating mechanisms of the mixture model
	\item experiments compare this mixture models to other models (ANM, PNL, IGCI, ECP
  and LiNGAM)
	\item They also did experiments on different noise standard deviations. They tested
	      the following cases: $\sigma = 0.01,\: 0.05$ and $0.1$. They concluded that the change
	      in $\sigma$ in this range does not significantly influence the performance of most
	      causal inference approaches.
	\item Clustering (compared to $k$-means, PCA-$k$m, GMM, SpeClu and DBSCAN) results rely
	      heavily on $\sigma$ and all approaches show a decreasing trend in avgARI as $\sigma$
	      increases. Their model (ANM-MM), however, is the most robust against large $\sigma$
\end{enumerate}

\parencite[][]{loh2013highdimensional}
\begin{enumerate}
        \item new framework for statistical estimation of DAGs when data are generated from a linear,
	      possibly non-Gaussian SEM.
	\item when the error variances are known or estimated to close enough preicision, the true
	      DAG is the unique minimizer of the score computed using the reweighted squared
	      $l_2$-loss
	\item The DAG structure of a lienar SEM is identifable whenever the additive errors
	      are homoscedastic
	\item errors may exhibit a certain degree of heteroscedasticity
\end{enumerate}

\parencite[][]{10.1093/biomet/ast043}
\begin{enumerate}
  \item Linear + gaussian + equal noise variance
  \item they tested their model with differently scaled noise variances\\
	$\to [1-a;1+a]$ where $a \in \{0, 0.1, \dots, 0.9\}$
\end{enumerate}


\parencite[][]{park2019identifiability}
\begin{enumerate}
  \item milder identifiability condition for linear gaussian models than \parencite[][]{10.1093/biomet/ast043}
  \item heterogeneous error variances $\to$ scale of error variances + edge weights
  \item variance ratio condition
  \item they conducted experiments with varying variances for linear gaussian structures
	i.e., $\sigma_j^2 \in [1,3]$
\end{enumerate}

\parencite[][]{shimizu2006linear}
\begin{enumerate}
  \item randomly selected variances of the disturbance variables
  \item but are not explicitly showing the effect of different noise levels
  \item not scale-invariant \parencite[][]{shimizu2014direct},$\to$ wrong ordering of variables 
	depending on scales or standard deviations of variables especially when they have a wide 
	range of scales
  \item However, scales are essentially not relevant to the ordering of variables. Though such bias 
	would vanish for large enough sample sizes, for practical sample sizes, an estimated ordering 
	could be affected when variables are normalized to make unit variance, and hence the 
	derivation of a reasonable ordering becomes quite difficult
\end{enumerate}

\parencite[][]{shimizu2014direct}
\begin{enumerate}
  \item new algorithm which does not require algorithmic parameters and is guaranteed to converge
	to the right solution within a small fixed number of steps if the data strictly follows the
	model
  \item randomly selected standard deviations of the external influences (noise) from $[0.5, 1.5]$
  \item $e_i \to$ various non-Gaussian distributions with zero mean and unit variance
  \item effect of different noise levels not explicitly shown
\end{enumerate}

\parencite[][]{5740928}
\begin{enumerate}
  \item Integer model: noise distribution random: $S \sim U(\{1,2,3,4,5\})$ determines the support
	$supp\;N = \{-S,\dots,S\}$
\end{enumerate}

\parencite[][]{mooij2009regression}
\begin{enumerate}
  \item Regression methods and independence tests
  \item How to choose the regression method if the noise distibution is unknown\\
	$\to$ they propose a regression method that makes no assumptions about the noise
        distribution, i.e., a method non-parametric with respect to the noise distribution
  \item In this paper they only assume the additive noise variable $E$ to have mean 0 and 
	independent of $X$
  \item $\to$ minimize the dependence between residuals $Y-f_{\alpha}(X)$ and the regressor $X$
  \item $\to$ replace the "log-likelihood" term in the common loss-function by the empirical 
	Hilbert Schmidt Independence Criterion estimator.
  \item ($E \sim Exp(1) - 1$ with mean 0)
  \item this regression method may prove to be more generally useful, in particular whenever the noise
	distribution is unknown
\end{enumerate}

\parencite[][]{kpotufe2014consistency}
\begin{enumerate}
  \item tests various additive noise models' statistical consistency of the inference
  \item general conditions under which common mehtods are consistent
  \item $\to$ to achive consistency, the independence test emplyed must detect more
	dependence between $N_y$ and $Y$ than between $N_x$ and $X$
  \item This papers analysis concerns procedures employing entropy-based independence measures
  \item $\to$ these test depends only on the marginal distributions of the random variables $X,Y$
	and functional residuals, and does not involve estimating joint distributions or conditionals,
	as is implicit in most independence tests
  \item In experiments they found out that for faster decreasing tail of the noise, the causal
	inference becomes better. (Their graph shows 0 - 1.2 and the previous sentence talks about
        1 -> 0. However, it seems that after 1.2 inference becomes better again. Though more data
	is needed to draw this conclusion). Kernel ridge regression tuned by cross-validation was used.
	They say that for properly tuned parameters, the selection of regression method does not
	seem to matter for the causal inference results.
  \item Convergence of causal inference is likeli faster if the noise has faster decreasing tail
  \item Assumption: Noise has bounded variance
  \item First consistency results for an existing family of procedures for causal inference under the
	Additive Noise Model; mild algorithmic requirements, and various distributional tail
        conditions which guarantee consistency
\end{enumerate}

\parencite[][]{mooij2016distinguishing}
\begin{enumerate}
  \item This work lists methods for causal discovery and performs benchmarks
  \item \textit{Additive Noise Models} and \textit{Information Geometric Causal Inference Models} are
	analysed
  \item CauseEffectPairs Dataset
  \item They only look at bivariate situations and the case with one confounder
  \item ANM: Any regression method can be used. However, they provide a theorem which states if a
	regression method is suitable enough or not. In this work they sticked to Gaussian Process
	Regression for nonparametric regression, using the GPML implementation. They used a squared
	exponential covariance function, constant mean function, and an additive Gaussian noise
	likelihood.
  \item Statistical tests for ANM: HSIC-Based Score, Entropy-Based Score, Gaussian Score,
	Empirical-Bayes Score, Minimum Message Length Scores, Minimizing HSIC Directly
  \item Simulated data $\to$ small noise function
\end{enumerate}

\parencite[][]{zhang2012identifiability}
\begin{enumerate}
  \item Post-Nonlinear Causal Model; ANM is a special case of PNL
  \item Provides all situations in which the PNL causal model is not identifiable; also proved
	by their work
\end{enumerate}












